Automatic Comment Generation via Multi-Pass Deliberation

Deliberation is a common and natural behavior in human daily life. For example, when writing papers or articles, we usually first write drafts, and then iteratively polish them until satisfied. In light of such a human cognitive process, we propose DECOM, which is a multi-pass deliberation framework for automatic comment generation. DECOM consists of multiple Deliberation Models and one Evaluation Model. Given a code snippet, we first extract keywords from the code and retrieve a similar code fragment from a pre-defined corpus. Then, we treat the comment of the retrieved code as the initial draft and input it with the code and keywords into DECOM to start the iterative deliberation process. At each deliberation, the deliberation model polishes the draft and generates a new comment. The evaluation model measures the quality of the newly generated comment to determine whether to end the iterative process or not. When the iterative process is terminated, the best-generated comment will be selected as the target comment. Our approach is evaluated on two real-world datasets in Java (87K) and Python (108K), and experiment results show that our approach outperforms the state-of-the-art baselines. A human evaluation study also confirms the comments generated by DECOM tend to be more readable, informative, and useful.

==> sec/2.background.tex <==

\section{Motivation}
\label{sec:background}
To illustrate the motivation of our approach, we select two representative examples from the Java and Python datasets, as shown in Figure \ref{fig:motivation}. Each example has a code-comment pair and three predictions generated by three state-of-the-art methods (i.e Re$^2$com \cite{DBLP:conf/kbse/WeiLLXJ20},  Rencos \cite{DBLP:conf/icse/ZhangW00020}, EditSum \cite{DBLP:conf/kbse/LiL000J21}). Comments highlighted in dashed and wavy lines are correct and incorrect, respectively.



Most existing comment generation methods adopt autoregressive models (e.g LSTM) and generate the comments with left-to-right decoding. Thus, these methods usually suffer from error propagation problems. Take the first example in Figure \ref{fig:motivation} into consideration. The three methods correctly predict the first two words ``calculates the", while mistakenly predict the third word ``weight", resulting in the following words conditioned on the wrong word being also wrongly generated. 
% Besides, the comments generated by Rencos and Editsum have repetition problem (the words "the" and "weight" are repeated twice in a row). 
This is mainly because these methods do not leverage the contextual information including both left and right parts when generating comments. 
% In fact, the contextual information is 
However, contextual information is crucial for natural language understanding \cite{DBLP:conf/emnlp/GuptaZLD19} and sequence generation tasks \cite{DBLP:conf/iwpc/BansalHM21}, which is also in line with human cognition.
For example, to write good documentation, we usually first write a complete draft, and then iteratively improve the draft based on the understanding of its context. When rewriting a specific part, we consider the overall information of the previous draft to determine which words are best for the current position, rather than just focusing on the left part. 
% This process will be repeated until we are satisfied with the current version of the documentation.
Similar to such human cognitive behaviors, if one model can rewrite the comment generated by EditSum, the third word ``weight" might be predicted correctly, since the ``weight" appears twice on the right side, indicating it is a keyword for this comment.
Based on this observation, we argue that the comment generation process can be an iterative process, and at each turn, the model can refine the generated comment from the prior turn by leveraging its context. 








% \input{table/motivation}
